Computing the Galois group of a polynomial over a $p$-adic field

We present a family of algorithms for computing the Galois group of a polynomial defined over a $p$-adic field. Apart from the "naive" algorithm, these are the first general algorithms for this task. As an application, we compute the Galois groups of all totally ramified extensions of $\mathbb{Q}_2$ of degrees 18, 20 and 22, tables of which are available online.

==> gg-sec-auxillary.tex <==
\section{Auxillary algorithms}
\label{gg-sec-auxillary}

A collection of algorithms used elsewhere in this article.

\subsection{Group embeddings}

\begin{algorithm}[Embed into direct product]
\label{gg-alg-embed-dp}
Given \(G \subgrp S_d\), returns \(s \in S_d\) and transitive \(G_1,\ldots,G_r\) such that \(\sum_i \deg G_i = d\) and \(G^s \subgrp G_1 \times \ldots \times G_r\).

The algorithm finds the image of the group acting on each of its orbits, then takes the direct product.

\begin{algorithmic}[1]
\State \(X_1=\{x_{1,1},\ldots\},\ldots,X_r \leftarrow \Orbits(G)\)
\State \(D \leftarrow G|_{X_1} \times \ldots \times G|_{X_r}\)
\State \(s \leftarrow\) permutation sending \(x_{i,j}\) to \(\sum_{i'<i} \abs{X_{i'}} + j\).
\State \Return \(D, s^{-1}\)
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[Embed into wreath product]
\label{gg-alg-embed-wr}
Given transitive \(G \subgrp S_d\), returns \(s\in S_d\) and primitive \(G_1,\ldots,G_r\) such that \(\prod_i \deg G_i = d\) and \(G^s \subgrp G_r \wr \ldots \wr G_1\).

We choose a minimal non-trivial block-partition of \(G\) and use this to embed \(G\) into \(A \wr B\) with the same block structure. We then recurse on \(B\).

Note that, unlike with the direct product case, there is not a canonical ``best'' (smallest) choice for the factors. Indeed, suppose we are given a group of the form \((A_1 \times \ldots \times A_e) \sdp B \subgrp S_d \wr S_e\), then we could embed it into \(A \wr B\) where \(A = \angles{A_1^{s_1},\ldots,A_e^{s_e}}\) for any \(s_i \in S_d\). Minimizing \(A\) is difficult. However, something cheap to compute is: for each \(i>1\), choose \(g_i \in G\) such that \(g_i(1) \in \{d(i-1)+1,\ldots,di\}\), and then reorder \((d(i-1)+1,\ldots,di)\) to \((g_i(1),\ldots,g_i(d))\) (i.e. let \(s_i\) permute \(j \mapsto g_i(j)-d(i-1)\)). If the best \(A\) is cyclic \(C_d\), this is guaranteed to find it.

\begin{algorithmic}[1]
\If{\(G\) is primitive}
  \State \Return \(G, id\)
\EndIf
\State \(P \leftarrow\) minimal partition of \(G\)
\State Fix an ordering \((B_1,\ldots,B_e)\) on \(P\)
\State Fix an ordering \((x_{i,1},\ldots,x_{i,d})\) on each \(B_i\)
\For{i = 1,\ldots,e}
  \State \(g_i \leftarrow\) an element of \(G\) such that \(g_i(x_{1,1}) = g_i(x_{i,1})\)
\EndFor
\State \(s \leftarrow\) the permutation \(g_i(x_{1,j}) \mapsto di+j\)
\State \(G' \subgrp S_d \wr S_e \leftarrow G^s\)
\State \(q : G' \to S_e\) the quotient
\State \(b : S_e \to S_d \wr S_e\) the canonical lift such that \(b(\sigma)(id+j)=\sigma(i)d+j\)
\State \(B \leftarrow q(G')\)
\State \(\cA \leftarrow \emptyset\)
\For{each generator \(g\) of \(G\)}
  \State \(g' \leftarrow g b(q(g))^{-1}\)
  \State \(\cA \leftarrow \cA \cup \{j \mapsto g'((i-1)d+j)-(i-1)d \suchthat i=1,\ldots,e\} \subset S_d\)
\EndFor
\State \(A \subgrp S_d \leftarrow \angles{\cA}\)
\State \((W_r,\ldots,W_1), s' \leftarrow\) embedding of \(B\) into a wreath product
\State \Return \((A,W_r,\ldots,W_1), sb(s')\)
\end{algorithmic}
\end{algorithm}

\subsection{Combinatorial}

\begin{algorithm}[Linear divisions]
\label{gg-alg-lindiv}
Given \(n \in \NN\) and multiset \(N \subset \NN\), returns all subsets \(M \subset N\) such that \(\sum M = n\).

We represent multisets of integers as a sorted sequence, with the largest element first. We loop over possible choices of the first division, and then recurse to assign the rest. An additional optional parameter \(L\) is such a sequence, and restricts any returned \(M\) to be at most \(L\) in the lexicographic ordering (i.e. if \(M \ne L\), then at the first place they disagree, \(M\) must be smaller). The default \(L\) is \(\{n\}\), which is no restriction.

\begin{algorithmic}[1]
\State \(S \leftarrow \emptyset\)
\For{distinct \(m_1 \in N\)}
  \If{\(m_1 \le \min(n, L_1)\)}
    \For{linear divisions \((m_2,\ldots)\) of \(n-m_1\) from \(N-\{m_1\}\) with limit \((L_2,\ldots)\) if \(m_1 = L_1\) or else limit \((m_1,m_1,\ldots)\)}
      \State Append \((m_1,m_2,\ldots)\) to \(S\)
    \EndFor
  \EndIf
\EndFor
\State \Return \(S\)
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[Rectangle divisions]
\label{gg-alg-recdiv}
Given \(w,h \in \ZZ\) and multiset \(A \subset \ZZ\), returns all multisets \(\{(w_i,\{h_{i,j}\})\}\) such that \(\sum_i w_i = w\), \(\sum_j h_{i,j} = h\) for each \(i\) and \(\{w_i h_{i,j} \suchthat i,j\} = A\). See \cref{gg-fig-recdiv}.

As with the previous algorithm, multisets are represented as sorted sequences. We loop over possible choices of the first division, and then recurse to assign the rest. Optional parameter \(L=(w_L,\{h_{L,j}\})\) limits the allowed divisions, with default \((w,\{h\})\).

\begin{algorithmic}[1]
\State \(S \leftarrow \emptyset\)
\For{distinct divisors \(w_1\) of some \(a \in A\)}
  \If{\(w_1 \le \min(w, w_L)\)}
    \For{linear divisions \((h_{1,1},h_{1,2},\ldots)\) of \(h\) from \(\{a/w_1 \suchthat a \in A, w_1 \mid a\}\) with limit \(h_{L,j}\) if \(w_1=w_L\) or else no limit}
      \For{rectangle divisions \(\{(w_2,\{h_{2,j}\}),\ldots\}\) of width \(w-w_1\), height \(h\), areas \(A-\{w_1h_{1,j}\}\), limit \((w_1,\{h_{1,j}\})\)}
        \State Append \((w_1,\{h_{1,j}\},\ldots)\) to \(S\)
      \EndFor
    \EndFor
  \EndIf
\EndFor
\State \Return \(S\)
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[Binning]
\label{gg-alg-binning}
Suppose we are given integers \((m_1,\ldots,m_r)\) and \((n_1,\ldots,n_s)\) such that we have \(m_i\) indistinguishable copies of some item \(i\), and \(n_j\) indistinguishable copies of some bin \(j\). A \define{binning} is some \((m'_1,\ldots,m'_r)\) with \(0 \leq m'_i \leq m_i\) for all \(i\). Suppose we are given a function \(V\) such that when \(V((m'_1,\ldots,m'_r),j)\) is true, we define the binning to be \define{valid for bin \(j\)}. Suppose we are given a function \(S\) such that whenever \((m'_1,\ldots,m'_r)\) is valid for bin \(j\) and \(0 \leq m''_i \leq m'_i\), then \(S((m''_1,\ldots,m''_r),j)\) is true. Such a binning is \define{semi-valid}. A \define{total valid binning} is a sequence of length \(s\), whose \(j\)th entry is a multiset of \(n_j\) valid binnings for bin \(j\), and such that all of these binnings sum to \((m_1,\ldots,m_r)\). This algorithm returns all total valid binnings.

Optionally, a \define{partial semi-valid binning} \(B\) can be given (like a total valid binning, except the binnings are only semi-valid and only sum to at most \(m_1,\allowbreak\ldots,\allowbreak m_r\)) and this algorithm only returns total valid binnings which extend it.

Optionally, a limit \(N\) can be given (defaulting to \(\infty\)) and this algorithm returns at most this many total binnings.

This algorithm works by choosing an item and considering all bins it could be added to. For each choice, we add this to the partial semi-valid binning, and recursively find all the total binnings extending it.

In order to avoid duplicated effort, we only add item \(i\) to a bin if either it makes the binning equal to the largest or exceed the largest, when comparing the \(i\)th entry in each binning.

Since items are assigned in order, they should be given to the algorithm in whatever order is likely to lead to a contradiction quickest (in terms of not being semi-valid). This usually means the ``largest'' items should come first, because these will ``fill'' the bins quicker.

\begin{algorithmic}[1]
\LineComment{Check semi-valid}
\If{\(B\) is not semi-valid}
  \State\Return \(\emptyset\)
\EndIf
\LineComment{Base case: nothing more to bin}
\If{\(m_i=0\) for all \(i\)}
  \If{\(B\) is a total valid binning}
    \State\Return \(\{B\}\)
  \Else
    \State\Return \(\emptyset\)
  \EndIf
\EndIf
\LineComment{General case}
\State \(\cR \leftarrow \emptyset\)
\State \(i \leftarrow \min \{i \suchthat m_i \ne 0\}\)
\State \(m_i \leftarrow m_i-1\)
\LineComment{Put an item \(i\) into one of the \(j\) bins}
\For{\(j=1,\ldots,k\)}
  \State \(B = \cB_i\) (a set of multiset binnings of size \(n_j\))
  \State \(B' \leftarrow\) the set of binnings in \(B\) with entry \(i\) set to 0
  \For{\(b' \in B'\)}
    \LineComment{Increase the highest value}
    \State \(m''_i \leftarrow\) the largest value of \(b_i\) among all \(b \in B\) agreeing with \(b'\) away from the \(i\)th entry
    \State \(b_0 \leftarrow\) \(b'\) with the \(i\)th entry set to \(m''_i\)
    \State \(b \leftarrow\) \(b'\) with the \(i\)th entry set to \(m''_i+1\)
    \State \(\cR \leftarrow \cR \cup\) all total valid binnings extending \(B\) with \(b_0\) replaced by \(b\) in \(B_i\)
    \LineComment{Increase the next one down}
    \State \(b_{-1} \leftarrow\) \(b'\) with the \(i\)th entry set to \(m''_i-1\)
    \If{\(b_{-1} \in B\)}
      \State \(\cR \leftarrow \cR \cup\) all total valid binnings extending \(B\) with \(b_{-1}\) replaced by \(b_0\) in \(B_i\)
    \EndIf
  \EndFor
\EndFor
\State \Return \(\cR\)
\end{algorithmic}
\end{algorithm}

